Sparse Probabilistic Graph Circuits

Deep generative models (DGMs) for graphs achieve impressively high expressive power thanks to very efficient and scalable neural networks. However, these networks contain non-linearities that prevent analytical computation of many standard probabilistic inference queries, i.e., these DGMs are considered \emph{intractable}. While recently proposed Probabilistic Graph Circuits (PGCs) address this issue by enabling \emph{tractable} probabilistic inference, they operate on dense graph representations with $\mathcal{O}(n^2)$ complexity for graphs with $n$ nodes and \emph{$m$ edges}. To address this scalability issue, we introduce Sparse PGCs, a new class of tractable generative models that operate directly on sparse graph representation, reducing the complexity to $\mathcal{O}(n + m)$, which is particularly beneficial for $m \ll n^2$. In the context of de novo drug design, we empirically demonstrate that SPGCs retain exact inference capabilities, improve memory efficiency and inference speed, and match the performance of intractable DGMs in key metrics.

==> figures/permuted_part_v2.tex <==
%%%%% graph
\node at ($(-16, -10) + (-4.0, 0)$) {(d) Graph $\pi\mathcal{G}$};


\node[circle,draw,fill=YlGn-E,inner sep=0pt,minimum size=1.2*\grid] (x1) at ($(-22, -8)$) {\scriptsize 3};
\node[circle,draw,fill=YlGn-B,inner sep=0pt,minimum size=1.2*\grid] (x2) at ($(-22, -4)$) {\scriptsize 1};
\node[circle,draw,fill=YlGn-J,inner sep=0pt,minimum size=1.2*\grid] (x3) at ($(-18, -8)$) {\scriptsize 4};
\node[circle,draw,fill=YlGn-G,inner sep=0pt,minimum size=1.2*\grid] (x4) at ($(-18, -4)$) {\scriptsize 2};

\draw[line width=0.25mm, draw=PuBu-F] (x1) to node[left]{} (x4);
\draw[line width=0.25mm, draw=PuBu-M] (x1) to node[left]{} (x3);
\draw[line width=0.25mm, draw=PuBu-H] (x3) to node[left]{} (x4);





%%%% permuted graph dense representation
\node at ($(d) + (2.0,0.0)$) {(e) Dense representation $\pi\mathbf{G}\coloneqq(\pi\mathbf{X}, \pi\mathbf{A})$};

% X

% EBJG
% BGEJ

\draw[draw=black,fill=YlGn-J] ($(d1) + (0,4)$) rectangle ($(d1) + (1,5)$) node[xshift=-0.5*\grid, yshift=-0.6*\grid] {};
\draw[draw=black,fill=YlGn-E] ($(d1) + (0,5)$) rectangle ($(d1) + (1,6)$) node[xshift=-0.5*\grid, yshift=-0.6*\grid] {};
\draw[draw=black,fill=YlGn-G] ($(d1) + (0,6)$) rectangle ($(d1) + (1,7)$) node[xshift=-0.5*\grid, yshift=-0.6*\grid] {};
\draw[draw=black,fill=YlGn-B] ($(d1) + (0,7)$) rectangle ($(d1) + (1,8)$) node[xshift=-0.5*\grid, yshift=-0.6*\grid] {};

\draw ($(d1) + (-0.9*\grid,7.5)$) node[label={[xshift=0.5*\grid, yshift=-0.85*\grid]$1$}] {};
\draw ($(d1) + (-0.9*\grid,4.5)$) node[label={[xshift=0.4*\grid, yshift=-0.85*\grid]$n$}] {};


% A
\draw[draw=c6,fill=c0] ($(d2) + (0,4)$) rectangle ($(d2) + (1,5)$) node[xshift=-0.5*\grid, yshift=-0.6*\grid] {};
\draw[draw=c6,fill=c0] ($(d2) + (3,4)$) rectangle ($(d2) + (4,5)$) node[xshift=-0.5*\grid, yshift=-0.6*\grid] {};

\draw[draw=c6,fill=c0] ($(d2) + (0,7)$) rectangle ($(d2) + (1,8)$) node[xshift=-0.5*\grid, yshift=-0.6*\grid] {};
\draw[draw=c6,fill=c0] ($(d2) + (3,7)$) rectangle ($(d2) + (4,8)$) node[xshift=-0.5*\grid, yshift=-0.6*\grid] {};

\draw[draw=c6,fill=c0] ($(d2) + (0,5)$) rectangle ($(d2) + (1,6)$) node[xshift=-0.5*\grid, yshift=-0.6*\grid] {};
\draw[draw=c6,fill=c0] ($(d2) + (0,6)$) rectangle ($(d2) + (1,7)$) node[xshift=-0.5*\grid, yshift=-0.6*\grid] {};

\draw[draw=c6,fill=c0] ($(d2) + (3,5)$) rectangle ($(d2) + (4,6)$) node[xshift=-0.5*\grid, yshift=-0.6*\grid] {};
\draw[draw=c6,fill=c0] ($(d2) + (3,6)$) rectangle ($(d2) + (4,7)$) node[xshift=-0.5*\grid, yshift=-0.6*\grid] {};

\draw[draw=c6,fill=c0] ($(d2) + (1,7)$) rectangle ($(d2) + (2,8)$) node[xshift=-0.5*\grid, yshift=-0.6*\grid] {};
\draw[draw=c6,fill=c0] ($(d2) + (2,7)$) rectangle ($(d2) + (3,8)$) node[xshift=-0.5*\grid, yshift=-0.6*\grid] {};

\draw[draw=c6,fill=PuBu-H] ($(d2) + (1,4)$) rectangle ($(d2) + (2,5)$) node[xshift=-0.5*\grid, yshift=-0.6*\grid] {};
\draw[draw=c6,fill=PuBu-M] ($(d2) + (2,4)$) rectangle ($(d2) + (3,5)$) node[xshift=-0.5*\grid, yshift=-0.6*\grid] {};


\draw[draw=c6,fill=PuBu-F] ($(d2) + (1,5)$) rectangle ($(d2) + (2,6)$) node[xshift=-0.5*\grid, yshift=-0.6*\grid] {};
\draw[draw=c6,fill=c0] ($(d2) + (1,6)$) rectangle ($(d2) + (2,7)$) node[xshift=-0.5*\grid, yshift=-0.6*\grid] {};
\draw[draw=c6,fill=c0] ($(d2) + (2,6)$) rectangle ($(d2) + (3,7)$) node[xshift=-0.5*\grid, yshift=-0.6*\grid] {};

% \draw[draw=c6,fill=c0] ($(d2) + (1,5)$) rectangle ($(d2) + (2,6)$) node[xshift=-0.5*\grid, yshift=-0.6*\grid] {};

\draw ($(d2) + (0,4)$) to node {} ($(d2) + (0,7)$);
\draw ($(d2) + (0,7)$) to node {} ($(d2) + (1,7)$);
\draw ($(d2) + (1,7)$) to node {} ($(d2) + (1,6)$);
\draw ($(d2) + (1,6)$) to node {} ($(d2) + (2,6)$);
\draw ($(d2) + (2,6)$) to node {} ($(d2) + (2,5)$);
\draw ($(d2) + (2,5)$) to node {} ($(d2) + (3,5)$);
\draw ($(d2) + (3,5)$) to node {} ($(d2) + (3,4)$);
\draw ($(d2) + (3,4)$) to node {} ($(d2) + (0,4)$);

\draw ($(d2) + (-0.9*\grid,7.5)$) node[label={[xshift=0.5*\grid, yshift=-0.85*\grid]$1$}] {};
\draw ($(d2) + (-0.9*\grid,4.5)$) node[label={[xshift=0.4*\grid, yshift=-0.85*\grid]$n$}] {};

\draw ($(d2) + (0.5,3.6*\grid)$) node[label={[xshift=0.0*\grid, yshift=-0.9*\grid]$1$}] {};
\draw ($(d2) + (3.5,3.6*\grid)$) node[label={[xshift=0.0*\grid, yshift=-0.9*\grid]$n$}] {};

\draw ($(d1) + (0.5,8.5)$) node {$\pi\mathbf{X}$};
\draw ($(d2) + (2.0,8.5)$) node {$\pi\mathbf{A}$};
% \draw ($(d2) + (2.5,2.5)$) node {$\mathbf{L}$};


\node at ($(e) + (4.0,0.0)$) {(f) Sparse representation $\pi\mathbf{G}\coloneqq(\pi\mathbf{V}, \pi\mathbf{E})$};

% Node tensor 
% 1st row

\draw[draw=black,fill=Oranges-D] ($(e1) + (0,2)$) rectangle ($(e1) + (1,3)$) node[xshift=-0.5*\grid, yshift=-0.6*\grid] {};
\draw[draw=black,fill=Oranges-G] ($(e1) + (1,2)$) rectangle ($(e1) + (2,3)$) node[xshift=-0.5*\grid, yshift=-0.6*\grid] {};
\draw[draw=black,fill=Oranges-J] ($(e1) + (2,2)$) rectangle ($(e1) + (3,3)$) node[xshift=-0.5*\grid, yshift=-0.6*\grid] {};
\draw[draw=black,fill=Oranges-M] ($(e1) + (3,2)$) rectangle ($(e1) + (4,3)$) node[xshift=-0.5*\grid, yshift=-0.6*\grid] {};

% 2nd row
\draw[draw=black,fill=YlGn-B] ($(e1) + (0,1)$) rectangle ($(e1) + (1,2)$) node[xshift=-0.5*\grid, yshift=-0.6*\grid] {};
\draw[draw=black,fill=YlGn-G] ($(e1) + (1,1)$) rectangle ($(e1) + (2,2)$) node[xshift=-0.5*\grid, yshift=-0.6*\grid] {};
\draw[draw=black,fill=YlGn-E] ($(e1) + (2,1)$) rectangle ($(e1) + (3,2)$) node[xshift=-0.5*\grid, yshift=-0.6*\grid] {};
\draw[draw=black,fill=YlGn-J] ($(e1) + (3,1)$) rectangle ($(e1) + (4,2)$) node[xshift=-0.5*\grid, yshift=-0.6*\grid] {};

\draw ($(e1) + (0.5,0.6*\grid)$) node[label={[xshift=0.0*\grid, yshift=-0.9*\grid]$1$}] {};
\draw ($(e1) + (3.5,0.6*\grid)$) node[label={[xshift=0.0*\grid, yshift=-0.9*\grid]$n$}] {};

\draw ($(e1) + (-0.8*\grid,2.6*\grid)$) node[label={[xshift=0.0*\grid, yshift=-0.9*\grid]$V^{\text{idx}}$}] {};
\draw ($(e1) + (-0.8*\grid,1.6*\grid)$) node[label={[xshift=0.0*\grid, yshift=-0.9*\grid]$V^{\text{type}}$}] {};


\draw ($(e1) + (2.0, 3.5)$) node {$\pi\mathbf{V}$};


% Edge Tensor
% 1st row  # D G J M
\draw[draw=black,fill=Oranges-J] ($(e2) + (0,2)$) rectangle ($(e2) + (1,3)$) node[xshift=-0.5*\grid, yshift=-0.6*\grid] {};
\draw[draw=black,fill=Oranges-M] ($(e2) + (1,2)$) rectangle ($(e2) + (2,3)$) node[xshift=-0.5*\grid, yshift=-0.6*\grid] {};
\draw[draw=black,fill=Oranges-M] ($(e2) + (2,2)$) rectangle ($(e2) + (3,3)$) node[xshift=-1.0*\grid, yshift=-0.5*\grid] {};

% 2nd row
\draw[draw=black,fill=Oranges-G] ($(e2) + (0,1)$) rectangle ($(e2) + (1,2)$) node[xshift=-0.5*\grid, yshift=-0.6*\grid] {};
\draw[draw=black,fill=Oranges-G] ($(e2) + (1,1)$) rectangle ($(e2) + (2,2)$) node[xshift=-0.5*\grid, yshift=-0.6*\grid] {};
\draw[draw=black,fill=Oranges-J] ($(e2) + (2,1)$) rectangle ($(e2) + (3,2)$) node[xshift=-1.0*\grid, yshift=-0.5*\grid] {};

% 3rd row
\draw[draw=black,fill=PuBu-F] ($(e2) + (0,0)$) rectangle ($(e2) + (1,1)$) node[xshift=-0.5*\grid, yshift=-0.6*\grid] {};
\draw[draw=black,fill=PuBu-H] ($(e2) + (1,0)$) rectangle ($(e2) + (2,1)$) node[xshift=-0.5*\grid, yshift=-0.6*\grid] {};
\draw[draw=black,fill=PuBu-M] ($(e2) + (2,0)$) rectangle ($(e2) + (3,1)$) node[xshift=-1.0*\grid, yshift=-0.5*\grid] {};

\draw ($(e2) + (0.5,-0.4*\grid)$) node[label={[xshift=0.0*\grid, yshift=-0.9*\grid]$1$}] {};
\draw ($(e2) + (2.5,-0.4*\grid)$) node[label={[xshift=0.0*\grid, yshift=-0.9*\grid]$m$}] {};

\draw ($(e2) + (-0.8*\grid,2.6*\grid)$) node[label={[xshift=0.0*\grid, yshift=-0.9*\grid]$E^{\text{idx}}_{s}$}] {};
\draw ($(e2) + (-0.8*\grid,1.6*\grid)$) node[label={[xshift=0.0*\grid, yshift=-0.9*\grid]$E^{\text{idx}}_{d}$}] {};
\draw ($(e2) + (-0.8*\grid,0.6*\grid)$) node[label={[xshift=0.0*\grid, yshift=-0.9*\grid]$E^{\text{type}}$}] {};


\draw ($(e2) + (1.5, 3.5)$) node {$\pi\mathbf{E}$};

